STEM: Unleashing the Power of Embeddings for Multi-task Recommendation

Multi-task learning (MTL) has gained significant popularity in recommender systems as it enables simultaneous optimization of multiple objectives. A key challenge in MTL is negative transfer, but existing studies explored negative transfer on all samples, overlooking the inherent complexities within them. We split the samples according to the relative amount of positive feedback among tasks. Surprisingly, negative transfer still occurs in existing MTL methods on samples that receive comparable feedback across tasks. Existing work commonly employs a shared-embedding paradigm, limiting the ability of modeling diverse user preferences on different tasks. In this paper, we introduce a novel Shared and Task-specific EMbeddings (STEM) paradigm that aims to incorporate both shared and task-specific embeddings to effectively capture task-specific user preferences. Under this paradigm, we propose a simple model STEM-Net, which is equipped with an All Forward Task-specific Backward gating network to facilitate the learning of task-specific embeddings and direct knowledge transfer across tasks. Remarkably, STEM-Net demonstrates exceptional performance on comparable samples, achieving positive transfer. Comprehensive evaluation on three public MTL recommendation datasets demonstrates that STEM-Net outperforms state-of-the-art models by a substantial margin. Our code is released at https://github.com/LiangcaiSu/STEM.

==> fig/conflict_analysis.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[tp!]
	\centering
	\includegraphics[width=0.97\linewidth]{figures/conflict.png}
	\caption{Construction of conflict datasets.}
	\label{fig:conflict}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> fig/embedding_dim.tex <==
\begin{figure}[t!]
	\centering  %图片全局居中
	\subfigbottomskip=0pt %两行子图之间的行间距
	\subfigcapskip=0pt %设置子图与子标题之间的距离
	\subfigure[Tiktok]{
		\includegraphics[width=0.48\linewidth]{figures/Tiktok_dim.pdf}}
	\subfigure[QK-Video]{
		\includegraphics[width=0.48\linewidth]{figures/QKVideo_dim.pdf}}
	% \subfigure[Tiktok]{
	% 	\includegraphics[width=0.48\linewidth]{figures/Tiktok_param.pdf}}
	% \subfigure[QK-Video]{
	% 	\includegraphics[width=0.48\linewidth]{figures/QKVideo_param.pdf}}
	% \subfigure[Comparison of performance under approximate number of parameters]{
	% 	\includegraphics[width=0.98\linewidth]{figures/embedding_dim_param.pdf}}
	% \subfigure[Average]{
	% 	\includegraphics[width=0.31\linewidth]{./images/param_exp_bar_avg.png}}
	\caption{The effect of embedding dimension. \# means "the number of".}
	\label{fig:embedding_dim}
\end{figure}

==> fig/embedding_exp.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t!]
	\centering
	\includegraphics[width=\linewidth]{figures/embedding_exp.pdf}
	\caption{AUC lift of STEM-Net variants compared to the Single-Task model of the task \texttt{Like} on task-overwhelming and
task-comparable samples.}
	\label{fig:embedding_exp}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> fig/gate.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[tp!]
	\centering
	\includegraphics[width=0.9\linewidth]{figures/gate_vis.png}
	\caption{The gate value of TOR on Tiktok and QKVideo.}
	\label{fig:gate_tiktok_qkvideo}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[tp!]
	\centering
	\includegraphics[width=0.97\linewidth]{figures/kuairand1k_gate.png}
	\caption{The gate value of TOR on KuaiRand1K.}
	\label{fig:gate_kuairand}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> fig/intro.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[tp!]
	\centering
	\includegraphics[width=0.8\linewidth]{figures/intro.png}
	\caption{An example of a user's preference relationship for different behaviours .}
	\label{fig:introduce}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> fig/latency_track.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t!]
	\centering
	\includegraphics[width=\linewidth]{figures/latency_track.pdf}
	\caption{Latency Track of MTL Models on KuaiRand1K.}
	\label{fig:latency_track}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> fig/param_embedding.tex <==
\begin{figure}[tp!]
	\centering  %图片全局居中
	\subfigbottomskip=0pt %两行子图之间的行间距
	\subfigcapskip=0pt %设置子图与子标题之间的距离
	% \subfigure[Tiktok]{
	% 	\includegraphics[width=0.48\linewidth]{figures/Tiktok_dim.pdf}}
	% \subfigure[QK-Video]{
	% 	\includegraphics[width=0.48\linewidth]{figures/QKVideo_dim.pdf}}
	\subfigure[Tiktok]{
		\includegraphics[width=0.48\linewidth]{figures/Tiktok_param.pdf}}
	\subfigure[QK-Video]{
		\includegraphics[width=0.48\linewidth]{figures/QKVideo_param.pdf}}
	% \subfigure[Comparison of performance under approximate number of parameters]{
	% 	\includegraphics[width=0.98\linewidth]{figures/embedding_dim_param.pdf}}
	% \subfigure[Average]{
	% 	\includegraphics[width=0.31\linewidth]{./images/param_exp_bar_avg.png}}
	\caption{The effect of parameter capacity.}
	\label{fig:parameter}
\end{figure}

==> fig/rep_vis.tex <==
\begin{figure}[tp!]
	\centering  %图片全局居中
	\subfigbottomskip=0pt %两行子图之间的行间距
	\subfigcapskip=0pt %设置子图与子标题之间的距离
	\subfigure[Single-Task(Finish)]{
		\includegraphics[width=0.48\linewidth]{CameraReady/LaTeX/figures/ST_finish_embeddings.pdf}}
	\subfigure[Single-Task(Like)]{
		\includegraphics[width=0.48\linewidth]{CameraReady/LaTeX/figures/ST_like_embeddings.pdf}}
	\subfigure[MMoE]{
		\includegraphics[width=0.48\linewidth]{CameraReady/LaTeX/figures/mmoe_shared_embeddings.pdf}}
	\subfigure[STEM-Net]{
		\includegraphics[width=0.48\linewidth]{CameraReady/LaTeX/figures/stem_embeddings.pdf}}
\caption{Visualization of Embeddings.}
	\label{fig:vis_embeddings}
\end{figure}

==> fig/representation.tex <==
\begin{figure}[tbp!]
	\centering  %图片全局居中
	% \subfigbottomskip=2pt %两行子图之间的行间距
	% \subfigcapskip=-5pt %设置子图与子标题之间的距离
	\subfigure[ST Finish Repr, -1 bin]{
		\includegraphics[width=0.3\linewidth]{figures/Finish, ST_-1.png}}
	\subfigure[MMoE Finish Repr, -1 bin]{
		\includegraphics[width=0.3\linewidth]{figures/Finish, MMoE_-1.png}}
	\subfigure[\ModelName Finish Repr, -1 bin]{
		\includegraphics[width=0.3\linewidth]{figures/Finish, TOR_-1.png}}
	\subfigure[ST Finish Repr, All]{
		\includegraphics[width=0.3\linewidth]{figures/Finish, ST_all.png}}
	\subfigure[MMoE Finish Repr, All]{
		\includegraphics[width=0.3\linewidth]{figures/Finish, MMoE_all.png}}
	\subfigure[\ModelName Finish Repr, All]{
		\includegraphics[width=0.3\linewidth]{figures/Finish, TOR_all.png}}
	\caption{Finish Task Representation Visualization}
	\label{fig:param_aliccp}
\end{figure}

\begin{figure}[tbp!]
	\centering  %图片全局居中
	% \subfigbottomskip=2pt %两行子图之间的行间距
	% \subfigcapskip=-5pt %设置子图与子标题之间的距离
	\subfigure[ST Like Repr, -1 bin]{
		\includegraphics[width=0.3\linewidth]{figures/Like, ST_-1.png}}
	\subfigure[MMoE Like Repr, -1 bin]{
		\includegraphics[width=0.3\linewidth]{figures/Like, MMoE_-1.png}}
	\subfigure[TOR Like Repr, -1 bin]{
		\includegraphics[width=0.3\linewidth]{figures/Like, TOR_-1.png}}
	\subfigure[ST Like Repr, All]{
		\includegraphics[width=0.3\linewidth]{figures/Like, ST_all.png}}
	\subfigure[MMoE Like Repr, All]{
		\includegraphics[width=0.3\linewidth]{figures/Like, MMoE_all.png}}
	\subfigure[TOR Like Repr, All]{
		\includegraphics[width=0.3\linewidth]{figures/Like, TOR_all.png}}
	\caption{Finish Task Representation Visualization}
	\label{fig:param_aliccp}
\end{figure}

==> sections/7_ethical.tex <==
\section{Ethical Considerations}
% https://www.acm.org/code-of-ethics
% 在本工作中，我们严格遵守道德规范。我们采用的三个公开数据集都是脱敏的，不会涉及到用户隐私的泄漏问题。 

In this study, we adhere strictly to ethical standards\footnote{\url{https://www.acm.org/code-of-ethics}} to ensure the integrity of our work. The three datasets utilized in our experiments, namely Tiktok, QK-Video, and KuaiRand, are all publicly available datasets that have undergone anonymization. We emphasize that the publication of this paper and the open-sourcing of our code do not infringe upon individuals' privacy.



==> tables/expert_abalation_study.tex <==
\begin{table}[]
\caption{The effect of experts on Tiktok}
\begin{tabular}{c|c|c|c|c}
\hline
Type & \#Specific Expert & Finish & Like & Average \\ \hline
\multirow{4}{*}{Linear} & 1 &  &  &  \\
 & 2 &  &  &  \\
 & 4 &  &  &  \\
 & 8 &  &  &  \\ \hline
\multirow{4}{*}{MLPs} & 1 &  &  &  \\
 & 2 &  &  &  \\
 & 4 &  &  &  \\
 & 8 &  &  &  \\ \hline
\end{tabular}
\end{table}

==> tables/latency.tex <==
\begin{table}[t]
    \small
    % \renewcommand\arraystretch{1}
    \centering
    \caption{Inference Latency on KuaiRand1K.}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|c|c|c|c}
    \toprule
\multirow{2}{*}{} & \multirow{2}{*}{Single-Task} & \multirow{2}{*}{MMoE} & \multirow{2}{*}{PLE} & \multicolumn{2}{c}{STEM (ours)} \\
                  &                          &   &                       & \multicolumn{1}{c}{$d$=8}      & $d$=16      \\ \midrule
        Avg.AUC & 0.8433 & 0.8437 & 0.8435 & 0.8464 & 0.8465 \\ 
        $\Delta$AUC & -- & +0.0004 & +0.0002 & +0.0031 & +0.0032 \\\hline
        Latency & 3.14$\times${8} ms & 10.15 ms & 10.99ms & 11.25ms & 11.31ms \\\bottomrule
    \end{tabular}
    }
    \label{tab:latency_tiktok} 
\end{table}


